LINX: A Language Driven Generative System for Goal-Oriented Automated Data Exploration

Data exploration is a challenging process in which users examine a dataset by iteratively employing a series of queries. While in some cases the user explores a new dataset to become familiar with it, more often, the exploration process is conducted with a specific analysis goal or question in mind. To assist users in exploring a new dataset, Automated Data Exploration (ADE) systems have been devised in previous work. These systems aim to auto-generate a full exploration session, containing a sequence of queries that showcase interesting elements of the data. However, existing ADE systems are often constrained by a predefined objective function, thus always generating the same session for a given dataset. Therefore, their effectiveness in goal-oriented exploration, in which users need to answer specific questions about the data, are extremely limited. To this end, this paper presents LINX, a generative system augmented with a natural language interface for goal-oriented ADE. Given an input dataset and an analytical goal described in natural language, LINX generates a personalized exploratory session that is relevant to the user's goal. LINX utilizes a Large Language Model (LLM) to interpret the input analysis goal, and then derive a set of specifications for the desired output exploration session. These specifications are then transferred to a novel, modular ADE engine based on Constrained Deep Reinforcement Learning (CDRL), which can adapt its output according to the specified instructions. To validate LINX's effectiveness, we introduce a new benchmark dataset for goal-oriented exploration and conduct an extensive user study. Our analysis underscores LINX's superior capability in producing exploratory notebooks that are significantly more relevant and beneficial than those generated by existing solutions, including ChatGPT, goal-agnostic ADE, and commercial systems.

==> introduction-old.tex <==

\section{introduction}
\label{sec:intro}

%dx is dififcult, therefore ade. 


%performed by data scientists and analysts in order to examine a dataset and extract insights from it.


Goal-oriented data exploration is the process in which analysts and data scientists examine the data to uncover insights and patterns that are relevant to a particular objective or question.

While this type of exploration is crucial, it has been scarcely addressed in previous work, which mainly focuses on the exploration of a \textit{new} datasets, assisting users in assessing its quality and understanding its nature~\cite{chanson2020traveling,chanson2022automatic,atenademo,atena_short,personnaz2021balancing,personnaz2021dora} -- often regardless of specific information needs.

 
 On the other hand, Large Language Models (LLMs) offer promising capabilities to facilitate the process of goal-oriented exploration, as models such as ChatGPT~\cite{chatgpt} excel in understanding instructions given in natural language, and generate coherent, human-like output. 
 Yet despite their promise, LLMs fundamentally lack the ability to interact deeply and repeatedly with the data itself, as a human analyst would have done. This limitation significantly hinders the LLM capability of directly discovering meaningful insights.  For illustration, consider the following example. 
\begin{example}
\label{ex:chat}
We asked ChatGPT to explore the Netflix Movies and TV Shows Dataset~\cite{netflixkaggle} (containing descriptive information on 9K Netflix titles, such as \textit{origin country, duration, genre, etc.}), with the goal of \textit{Finding a country with different viewing habits than the rest of the world}.

Note that this compound exploratory goal cannot be answered via a single analytical operation or an SQL query, as it requires to both \textit{discover} such a country that deviates with respect to several attributes in the data, then to build an adequate exploratory path that showcases the evidence for the discovery —such as aggregating on the deviating attributes and comparing between the atypical country and the rest of the world.



Given a prompt containing a description of the dataset and the goal (the full prompt and answer are available in our Github repository~\cite{our_github_repository}), the LLM outputs a sequence of exploratory operations, implemented in Pandas~\cite{pandas}, alongside the following description of its logic: \textit{We first filter the dataset to separate TV shows and movies. Then, we calculate the global percentage of TV shows and movies by dividing the number of TV shows/movies by the total number of entries in the dataset. 
Next, we group the dataset by country and calculate the percentage of TV shows and movies for each country.
We then compare the country percentages to the global percentages and identify countries with a difference of more than 10\%.} %\qed

While the LLM successfully understands that a country is to be compared to the rest of the world, see that it chose to focus its comparison solely on the attribute `Type' (Movie/TV-Show), thus using a fixed, predefined notion of atypical country:  having a 10\% deviation in the ratio of movies to TV-shows. Yet, there are 10 other attributes ignored by the LLM, and hundreds of different alternative ways to define an atypical country in the data. The most suitable one should be discovered by examining the utility and relevance of multiple different alternative exploration paths. 





%it uses a predefined notion of what is an atypical country (having a 10\% deviation in the ratio of movies to TV-shows). Instead, this definition should have been discovered using a repeated interaction with the data, examining multiple countries and comparing them to the rest of the world w.r.t. different attributes. Unfortunately, language models inherently lack the ability to deeply examine the data, i.e., by employing a multitude of exploratory operations, examining the utility and interestingness of their output and use it to further guide the continuation of the exploratory process.  \amit{as you can see, it chose to focus on one specific attribute (type). This is a preconcived notion, since further interactive exploration shows that there are other aspects. Chat's answer is limited..  There are other attribtues and aspects. It discovered 30 countries that fits the description. }
\end{example}

Unfortunately, language models inherently lack the ability to employ a multitude of exploratory operations, examining the utility and interestingness of their output and use it to further guide the continuation of the exploratory process.



To this end, we introduce \system{}, a \textit{Language-driven generative system for goal-oriented exploration}. Given a dataset and a goal description in natural language, \system{} generates a \textit{personalized} exploratory session tailored to the goal at hand. \system{} overcomes the LLM inability to interact with the data by segregating the generative process into \textit{planning} and \textit{execution}. We first harness the LLM's ``analytical mind'' to deduce a set of specifications for the exploratory process based on the user's definition of their analytical task. The exploratory specifications and dataset are then given to a data-driven, Constrained Deep Reinforcement Learning (CDRL) engine, that can actually interact with the input dataset, observe the output of its own analytical operations, then gauge their utility and relevance in order to refine the exploratory process.

%In an intelligent trial-and-error manner, the CDRL engine discovers a useful exploration notebook that complies with the user's analytical task. 







\amit{stop reading}






Data exploration constitutes a crucial yet formidable process for data scientists and analysts. When confronted with an analytical task or inquiry \tomer{I'm assuming that analytical task and inquiry are standard jargon, right?} concerning a dataset, users sequentially execute exploratory queries, such as filtering and grouping, to extract pertinent insights for their task.
One of the most effective methods to kickstart this intricate process is to examine existing \textit{data exploration notebooks}~\cite{rule2018exploration,kery2018story,perkel2018jupyter}—curated, illustrative exploratory sessions crafted by other data scientists on the same dataset, often shared on collaborative online platforms like Kaggle, Google Colab, or Github. However, in many cases, such notebooks are unavailable or nonexistent. 
In a previous work, we introduced ATENA~\cite{atena_short}—a system designed to automatically generate general-purpose exploration notebooks based on an input dataset. 
Nonetheless, general-purpose notebooks may be inadequate, since users may have distinct information needs stemming from diverse analysis tasks. To address this, autogenerated notebooks must be far more personalized. 

To this end, we introduce \system{}, a \textit{Language-driven generative data exploration system}. Given a dataset and an analytical task description in natural language, \system{} generates a \textit{personalized} exploratory notebook tailored to the user's specified task.



 In the notebook composition process, \system{} utilizes Large Models (LLMs), renowned for their exceptional generative capabilities, such as writing code snippets and even processing small data amounts~\cite{gpt35,openai2023gpt4,openai_advanced_data_analysis}. However, we make an important observation: LLMs cannot generate optimal exploration notebooks \textit{directly}, because \textit{they lack the ability to comprehensively interact with the data itself}. Correspondingly, as we assert through our experimental evaluation, notebooks composed directly by ChatGPT yield notably fewer relevant insights compared to those generated by \system{}. 
This deficiency arises because meaningful insights are often discovered through continuous refinement of the analytical process, and examination of numerous exploratory paths until discoveries are made.


%While LLMs demonstrate promising generative capabilities, including the ability to generate code snippets and process small data amounts effectively \cite{openai_advanced_data_analysis}, \textit{they lack the ability to truly interact with the data itself}. Correspondingly, as we assert through our experimental evaluation, notebooks composed directly by ChatGPT yield significantly fewer relevant insights compared to those generated by \system{}. 

\system{} overcomes this limitation of LLMs by segregating the generative process into \textit{planning} and \textit{execution}. We first harness the LLM's ``analytical mind'' to deduce a set of specifications for the exploratory process based on the user's definition of their analytical task. The exploratory specifications and dataset are then given to a data-driven, Constrained Deep Reinforcement Learning (CDRL) engine, that can actually interact with the input dataset and observe the output of its own analytical operations. In an intelligent trial-and-error manner, the CDRL engine discovers a useful exploration notebook that complies with the user's analytical task. 

Correspondingly, we face two major research challenges:

%


%\amit{
%An ideal exploration notebook exhibits a sequence of semantically connected analytical operations, while maintaining a coherent narrative and structure~\cite{kery2018story}. Constructing such notebooks requires iterative interactions with the data, uncovering interesting subsets or aggregations through trial and error, and subsequently exploring them in successive operations. 
%}


%\amit{During the planning phase, our LLM-based \textit{exploration plan generator} determines which elements in the notebook can be immediately derived and which should be discovered in a data-driven manner.}





%Recently, Large Language Models (LLMs) such as ChatGPT~\cite{gpt35} and GPT-4~\cite{openai2023gpt4} demonstrate superb generative capabilities, including the ability to generate code snippets and process small data amounts effectively \cite{openai_advanced_data_analysis} 


%While LLMs demonstrate promising generative capabilities, including the ability to generate code snippets and process small data amounts effectively \cite{openai_advanced_data_analysis}, \textit{they lack the ability to truly interact with the data itself}. Correspondingly, as we assert through our experimental evaluation, notebooks composed directly by ChatGPT yield significantly fewer relevant insights compared to those generated by \system{}. 
%This deficiency arises because meaningful insights often emerge through a continuous refinement of the analytical process, and examination of numerous exploratory paths until discoveries are made.



%To this end, we present \system{}, a Language-drIven geNerative data eXploration system.  
%a new system for generating \textit{personalized}, \textit{task-relevant} exploration notebooks.
%Given a dataset and an analytical task description provided by the user in natural language, \system{} uses a twofold solution for generating a personalized exploratory notebook: First, it uses a (1) Large Language Model (LLM) component for generating an \textit{exploration plan}, based on the analytical task description. This LLM-generated plan is then used to guide a (2) 

%\amit{first describe the observation than the two challenges.}

\vspace{1mm}

\noindent\textbf{C1. Deriving an exploration plan using an LLM.} 
An ideal exploration notebook exhibits a sequence of semantically connected analytical operations, while maintaining a coherent narrative and structure~\cite{kery2018story}. 
Whether crafted by a human analyst or an AI agent, the process involves iterative interactions with the data, uncovering interesting subsets or aggregations through trial and error, and subsequently exploring them in successive operations. 

The primary challenge lies in determining which elements in the desired exploration notebook can be immediately derived from the user's task description and which should be discovered in a data-driven manner.

We address this challenge by, first, introducing a specification language for data exploration processes (\lang{}). \lang{} allows specifying desired fragments in the output sequence of analytical operations, shaping its structure, and crucially, defining how to contextually link individual operations. \oz {need to give motivation here why we need LDX before explaining our solution to generate it.} \oz {Alternatively, we can also introduce our novel pandas-like input, and then explain that we plug-in it to the DRL engine via LDX }
However, directly deriving \lang{} specifications presents an additional challenge for an LLM, primarily due to the absence of pertinent information in its training data. We tackle this issue by employing a two-stage chained prompt approach: In the first stage, we generate template Python Pandas~\cite{openai2023gpt4} code, a format highly prevalent in LLM training sources such as Stackoverflow and Github\cite{openai2023gpt4}. The resulting code template is then translated to \lang{} through a subsequent prompt.









%The exploration plan is expressed in a novel Specification Language for Data Exploration (\lang{}). \lang{} allows specifying desired fragments in the output sequence of analytical operations, shaping its structure, and defining how to contextually link individual operations. 


%\noindent\textbf{The data-driven limitation of LLMs (or: why LLMs cannot generate optimal exploration notebooks \textit{directly}).} 



%This is because meaningful insights are often discovered by a continuous refinement of the analytical process, trying numerous explroation paths. 

%\system{} overcomes this limitation of LLMs by segregating the generative process into \textit{planning} and \textit{execution}. We harness the LLM's ``analytical mind'' to deduce a set of specifications for the exploratory process based on the user's definition of their analytical task. During the planning phase, our LLM-based \textit{exploration plan generator} determines which elements in the notebook can be immediately derived and which should be discovered in a data-driven manner.



%Deriving exploration plans poses a challenge for an LLM, primarily due to the absence of pertinent information in its training data. We address this issue by employing a two-stage chained prompt. In the first stage, we generate template Python Pandas~\cite{openai2023gpt4} code, a format highly prevalent in LLM training sources such as Stackoverflow and Github\cite{openai2023gpt4}. The resulting code template is then translated to \lang{} through a subsequent prompt.



%Deriving the \lang{} specifications from the user-provided task is performed via our LLM-based \textit{exploration plan generator}. To overcome the lack of \lang{} in the LLM training data, we use a two-stage chained prompt, first generating template Python Pandas code (highly prevalent in LLM training sources such as Stackoverflow and Github). The resulting code template is translated to \lang{} via a subsequent prompt. 



%The \lang{} plan's execution is carried out by the \system{} CDRL engine, which generates a useful sequence of analytical operations on the input dataset in accordance with the provided specifications, as described below.







%






%We validate this claim in our experimental evaluation, showing that notebooks constructed directly via ChatGPT yield significantly less relevant insights than the ones generated by \system{}.

%\system{} overcomes this LLM limitation by separating the exploratory process generation to \textit{planning} and \textit{execution}.  
%We exploit the LLM's ``analytical mind'' in order to derive a set of specifications to the exploratory process that stem from the user's definition of the analytical tasks, then a data-driven CDRL engine to execution the plan and discover a useful sequence of analytical operations, as described below. 

%The exploration plain is given in a novel Specification Language for Data E\textit{X}ploration (\lang{}). \lang{} allows to partially (or fully) specify a sequence of analytical operations, define its structure, and also provide \textit{continuity} definitions that contextually connect between the individual  operations.




%producing a ``good'' exploration notebook is a challenge for the LLM as 







%Naturally, a useful interface should allow (partially) specifying the notebook's structure and operations, but the key challenge is to facilitate \textit{contextual} specifications that interconnect the operations in the notebook.
%As shown in~\cite{kery2018story}, ``good'' exploration notebooks have a \textit{clear, continuous narrative and structure}, in which the individual operations are semantically connected.

%To our knowledge, previous work has not dealt with answering users' information needs from a \textit{full sequence} of analytical operations. 
%We therefore devise a novel Specification Language for Data E\textit{X}ploration (\lang{}). \lang{} allows users to partially (or fully) specify the notebook's operations, structure, and also provide \textit{continuity} definitions that contextually connect between the individual analysis operations.




\vspace{1mm}
%\noindent\textbf{Taming DRL: How to guide a DRL agent to produce \textit{personalized} exploratory notebooks}

\noindent\textbf{C2. Guiding a DRL Agent to Produce \textit{Personalized} Exploratory Notebooks Using the Exploration Plan.} 
In our prior work~\cite{atena_short}, we demonstrated that generating useful analytical sessions (although task-agnostic) is a challenging computational task but feasible with a dedicated deep reinforcement learning scheme. In this approach, a neural-network-based agent iteratively interacts with the input dataset to uncover valuable exploration paths. However, generating useful notebooks that are compliant with the input exploration plan is highly non-trivial, given that only a small fraction of the vast space of possible exploratory paths adheres to the specifications. This poses a reward-sparsity problem, a well-known challenge in reinforcement learning~\cite{mataric1994reward}.

To address this challenge, we draw inspiration from prior work in \textit{constrained deep reinforcement learning} (CDRL)~\cite{saunders2017trial,dalal2018safe}, where the neural network agent is specifically designed to handle additional requirements, such as safety constraints~\cite{garcia2015comprehensive}. 
In \system{}, both the dataset and the \lang{} exploration specifications are provided as input to the CDRL engine. Our CDRL engine is built on top of the generic exploration framework of~\cite{atena_short}, augmenting it with two main novel components:
(1) a \textit{specification-compliance} reward scheme that integrates multiple feedback signals, encouraging the agent to initially generate notebooks with a correct \textit{structure} and then make further adjustments to operation parameters. (2) An adaptive, \textit{specification-aware neural network} that derives its final structure from the \lang{} specifications, thereby prompting the agent to ``explore'' the space of compliant operations with a higher probability.


















%For illustration, consider the following example.


%\paragraph*{Example Scenario}


\begin{comment}
\begin{figure}
%\begin{minipage}{\columnwidth}
\begin{adjustbox}{max width=\columnwidth}

\small 
\centering
\ttfamily
    \begin{tabular}{|l|l|l|c|c|l|l|}
    \hline
    \rowcolor{gray!40}
    \textbf{type} & \textbf{title} & \textbf{country} & $\ldots$ & \textbf{dur.} & \textbf{genre} & \textbf{rating} \\
    \hline
    Movie & Bareilly Ki.. & India & $\ldots$ & 110 & Intl. & TV-14 \\
    TV & Imposters & USA & $\ldots$ & 2 & Comedies & TV-MA  \\
    Movie & Pulp Fiction & USA & $\ldots$ & 154 & Classic & R  \\ 
    TV & Thomas \& Fri.. & UK & $\ldots$ & 2 & Kids & TV-Y  \\ 
    $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ & $\ldots$ \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{-4mm}
\caption{Netflix Dataset Sample}
\label{fig:netflix_sapmle}
\vspace{-5mm}

%\end{minipage}
\end{figure}

\end{comment}





%\vspace{-1mm}
%This example demonstrates the usefulness in reviewing personalized exploration notebooks, relevant to the task at hand. However, \textit{automatically} generating such notebooks requires overcoming 
%two major research challenges:
%While basic elements of the \system{} engine utilize the generic exploration framework of~\cite{atena_short}, we face three major research challenges:


\vspace{2mm}

To empirically assess \system{}, we conducted an extensive set of experiments. Initially, we present results using a new benchmark dataset comprising 182 analytical tasks and corresponding \lang{} plans. Our LLM-based plan generator demonstrates high performance, successfully generating correct exploration plans even when both the analytical task and dataset are unseen in the prompts.

Next, we carried out a comprehensive user study involving 30 participants to evaluate the relevance and overall quality of \system{} notebooks. The results are highly positive: Notebooks generated by \system{} not only receive higher ratings for usefulness and relevance compared to baselines like ChatGPT and ATENA but also significantly aid users in completing analytical tasks, providing 3-5 times more relevant insights.
Finally, we examined the effectiveness of \system{}'s CDRL engine, demonstrating that the convergence and performance of \system{} are comparable to ATENA~\cite{atena_short}. This is noteworthy, considering \system{}'s more complex reward scheme and neural network architecture, used for handling the custom exploration specifications.

%A demo paper partially describing the \lang{} language and CDRL engine has been recently published~\cite{lipman2023atena}, yet it focuses on a UI that wraps \lang{}, in which users are required to compose the specifications by themself, as opposed to \system{} in which the users just provide a description of the analytical task. 

\vspace{1mm}
A recent demo paper~\cite{lipman2023atena} briefly introduces \lang{} and the CDRL engine, but with a focus on a web interface for manual specification composition (rather than a description of the task, as in \system{}). %This differs from \system{}, where users simply provide a task description.







%To empirically evaluate \system{}, we performed an extensive experiments set: We first show, via a new benchmark of 182 analytical tasks~\cite{our_github_repository}, that our LLM-based exploration plan generator obtains high performance, able to successfully generate \lang{} plans even when both the analytical task and dataset are unseen (i.e., provided in the few-shots prompt). 

%We then conducted a vast user study with 30 participants to gauge the relevance and overall quality of the \system{} notebook. our results are highly positive: notebooks generated by \system{} are not only rated as far more useful and relevant than baselines such as ATENA and ChatGPT, but they also substantially assist users in completing analytical tasks, providing 3-5X more relevant insights. Last, we examined the performance of \system{} CDRL engine, demonstrating that the convergence and performance of \system{} are on par with ATENA~\cite{atena_short}, despite its more complex reward scheme and neural network architecture. 

%as well as a performance and ablation study, assessing the convergence process of \system{} compared to ATENA~\cite{atena_short}. Our experimental results are highly positive: (1) users are finding the specification UI convenient and easy-to-use; (2) notebooks generated by \system{} are not only rated as far more useful and relevant than baselines such as ATENA and ChatGPT, but they also substantially assist users in completing analytical tasks, providing 3-5X more relevant insights; and last (3) the performance and convergence of \system{} are on par with ATENA, despite its more complex reward scheme and neural network architecture. 



%\noindent\textbf{C3. \textit{How to empirically validate the usability of \system{}?} }

%There are multiple factors in \system{} that are needed to be  evaluated: First, we need to assess the usability and ease-of-use of the specification interface, and gauge whether users are willing to use \system{} as a part of their analytical workflows. To that end we conduct a \textit{formative evaluation}, in which users interact with the \system{} UI and estimate their confidence and willingness in using it for various analytical tasks. 
%The second factor is the relevance and overall quality of the output notebooks. We evaluate it via an elaborate \textit{summative study} where users inspect notebooks generated by \system{} as well as baselines such as ATENA~\cite{atena_short} and notebooks generated by ChatGPT~\cite{chatgpt}. We measure both their subjective opinion (rating) and also their objective success in completing analytical tasks. 
%The last factor is performance, in which we need to show that although \system{} has a more complex reward scheme and CDRL architecture, its convergence and running times are on par with the task-agnostic ATENA~\cite{atena_short} System. 

%Our experimental results are highly positive: (1) users are finding the specification UI as convenient and not-too-difficult; (2) the notebooks generated by \system{} are rated far more relevant than the baselines, as well as practically assist users in completing analytical tasks better (3-5X more relevant insights); and last (3) the performance and convergence of \system{} stay similar to those of  ATENA, despite its more complex architecture. 


\vspace{2mm}
\textit{Paper Outline.}
We begin with a brief overview and illustration of our system workflow (§\ref{sec:prelim}). We then introduce the \lang{} specification language and its corresponding verification engine (§\ref{sec:language}). Next, we describe  the exploration plan generator (§\ref{sec:ldx_llm}) and  our CDRL engine (§\ref{sec:engine}). Subsequently, we detail our experimental results (§\ref{sec:experiments}), review related work (§\ref{sec:related}), and conclude with final remarks (§\ref{sec:conclusion}).


%We begin with a brief overview and exemplify our system workflow (§\ref{sec:prelim}). Next, we present the \lang{} specification language and its verification engine (§\ref{sec:language}).
%We then describe the exploration plan generator (§\ref{sec:ldx_llm}), and our CDRL engine (§\ref{sec:engine}). Afterwards, we describe our experiments (§\ref{sec:experiments}), review related work (§\ref{sec:related}), and provide final remarks in (§\ref{sec:conclusion}).  


%then describe our CDRL framework of \system{}: the compliance reward scheme (§\ref{sec:reward}) and specification-aware neural network (§\ref{sec:network}). Afterwards, we describe our experiments (§\ref{sec:experiments}), review related work (§\ref{sec:related}), and provide final remarks in (§\ref{sec:conclusion}).  



%In addition, we fully publish our source code~\cite{our_github_repository}, inviting researchers and practitioners to use our prototype system implantation. 


%We show that relatively to these tools, users who used \system{} obtained more than 3 times more relevant insights than the alternatives.  

%We show that \system{} successfully generates compatible sessions, rated highly relevant in a user study. We also discuss the meaningful and compound insights that users gain from viewing the data stories produced by \system{}. 

%\amit{insert here a paragraph on the related work - many works do similar things but not the same, see section related for an elaborate discussion., as well as the baselines in the experiments}







%\paragraph*{Paper Outline}

%We begin by a brief, preliminary overview of the basic DRL environment for data exploration in Section \ref{sec:prelim} (\amit{and the languages}). We then describe our framework as follows:
%In Section~\ref{sec:language} we present \lang{}, the specification language for exploratory sessions . Then, our specification-compliance reward scheme is described in Section~\ref{sec:reward}. Our specification-aware neural network architecture is then detailed in Section~\ref{sec:network_arch}.
%Our experimental evaluation is brought in Section~\ref{sec:experiments},
%the experimental evaluation in Section~\ref{sec:experiments} and finally, related work and conclusion are in Section~\ref{sec:related} and~\ref{sec:conclusion}. 








\begin{figure*}[t]
\vspace{-6mm}
    \includegraphics[width=\linewidth]{figures/linx_arch.pdf}
    \vspace{-6mm}
    \caption{\system{}\includegraphics[width=0.015\textwidth]{figures/huggingcat.png} 
Workflow Overview  } %\faCat

%\amit{fix the != + extra space,change name to plan generator, take the new notebook fig with number fix} \oz{consider changing placeholders in pandas template to CV, e.g <X> to ?(<X>).*}. Also the convertion from this template to his LDX might not be clear since they different ordered and the template has one comparison and not two as in the LDX
    \label{fig:ap_workflow}
\end{figure*}


















